Experimental Validation of a Microscopic Ellipsoidal Particle Model Immersed in Fluid Flow

A simulation of ellipsoidal particles inside a fluid flow is presented and validated from our own lab size experiments where data has been recorded using a camera set-up and post-processing of the pictures. The model is based on Jeffery's equation, where the orientation and position of the particles are influenced by the surrounding fluid. Additionally, particle-particle interaction and particle-wall interaction are taken into account.

==> pictures/tikz/ell_exp/groupplots/ell_exp-block-1.tex <==
\nextgroupplot[
xmin=0,
xmax=29,
ymin=0,
ymax=5,
%view={0}{90},
axis equal,
xlabel=$x$,
ylabel=$y$,
title=\tikztitle{Time t= 0.0}],
\addplot+[green,no marks,quiver={u=\thisrow{u},v=\thisrow{v},scale arrows=  0.03000000},-stealth] table {\relincludepath Data/Datafile-1.txt};
\fill[white] (axis cs: 2.500000e+00,2.250000e+00) rectangle (axis cs: 2.650000e+01,2.750000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 0,0) -- (axis cs: 29,0);
\draw[-,red,line width=0.5mm] (axis cs: 29,5) -- (axis cs: 29,0);
\draw[-,red,line width=0.5mm] (axis cs: 0,5) -- (axis cs: 29,5);
\draw[-,red,line width=0.5mm] (axis cs: 0,5) -- (axis cs: 0,0);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.250000e+00) -- (axis cs: 2.650000e+01,2.250000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.650000e+01,2.750000e+00) -- (axis cs: 2.650000e+01,2.250000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.750000e+00) -- (axis cs: 2.650000e+01,2.750000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.750000e+00) -- (axis cs: 2.500000e+00,2.250000e+00);
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-2.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-3.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-4.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-5.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-6.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-7.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-8.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-9.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-10.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-11.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-12.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-13.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-14.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-15.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-16.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-17.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-18.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-19.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-20.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-21.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-22.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-23.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-24.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-25.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-26.txt};


==> pictures/tikz/ell_exp/groupplots/ell_exp-block-2.tex <==
\nextgroupplot[
xmin=0,
xmax=29,
ymin=0,
ymax=5,
%view={0}{90},
axis equal,
xlabel=$x$,
ylabel=$y$,
title=\tikztitle{Time t= 2.5}],
\addplot+[green,no marks,quiver={u=\thisrow{u},v=\thisrow{v},scale arrows=  0.03000000},-stealth] table {\relincludepath Data/Datafile-27.txt};
\fill[white] (axis cs: 2.500000e+00,2.250000e+00) rectangle (axis cs: 2.650000e+01,2.750000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 0,0) -- (axis cs: 29,0);
\draw[-,red,line width=0.5mm] (axis cs: 29,5) -- (axis cs: 29,0);
\draw[-,red,line width=0.5mm] (axis cs: 0,5) -- (axis cs: 29,5);
\draw[-,red,line width=0.5mm] (axis cs: 0,5) -- (axis cs: 0,0);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.250000e+00) -- (axis cs: 2.650000e+01,2.250000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.650000e+01,2.750000e+00) -- (axis cs: 2.650000e+01,2.250000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.750000e+00) -- (axis cs: 2.650000e+01,2.750000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.750000e+00) -- (axis cs: 2.500000e+00,2.250000e+00);
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-28.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-29.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-30.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-31.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-32.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-33.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-34.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-35.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-36.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-37.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-38.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-39.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-40.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-41.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-42.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-43.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-44.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-45.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-46.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-47.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-48.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-49.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-50.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-51.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-52.txt};


==> pictures/tikz/ell_exp/groupplots/ell_exp-block-3.tex <==
\nextgroupplot[
xmin=0,
xmax=29,
ymin=0,
ymax=5,
%view={0}{90},
axis equal,
xlabel=$x$,
ylabel=$y$,
title=\tikztitle{Time t= 7.5}],
\addplot+[green,no marks,quiver={u=\thisrow{u},v=\thisrow{v},scale arrows=  0.03000000},-stealth] table {\relincludepath Data/Datafile-53.txt};
\fill[white] (axis cs: 2.500000e+00,2.250000e+00) rectangle (axis cs: 2.650000e+01,2.750000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 0,0) -- (axis cs: 29,0);
\draw[-,red,line width=0.5mm] (axis cs: 29,5) -- (axis cs: 29,0);
\draw[-,red,line width=0.5mm] (axis cs: 0,5) -- (axis cs: 29,5);
\draw[-,red,line width=0.5mm] (axis cs: 0,5) -- (axis cs: 0,0);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.250000e+00) -- (axis cs: 2.650000e+01,2.250000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.650000e+01,2.750000e+00) -- (axis cs: 2.650000e+01,2.250000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.750000e+00) -- (axis cs: 2.650000e+01,2.750000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.750000e+00) -- (axis cs: 2.500000e+00,2.250000e+00);
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-54.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-55.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-56.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-57.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-58.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-59.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-60.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-61.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-62.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-63.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-64.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-65.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-66.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-67.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-68.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-69.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-70.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-71.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-72.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-73.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-74.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-75.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-76.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-77.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-78.txt};


==> pictures/tikz/ell_exp/groupplots/ell_exp-block-4.tex <==
\nextgroupplot[
xmin=0,
xmax=29,
ymin=0,
ymax=5,
%view={0}{90},
axis equal,
xlabel=$x$,
ylabel=$y$,
title=\tikztitle{Time t= 10.0}],
\addplot+[green,no marks,quiver={u=\thisrow{u},v=\thisrow{v},scale arrows=  0.03000000},-stealth] table {\relincludepath Data/Datafile-79.txt};
\fill[white] (axis cs: 2.500000e+00,2.250000e+00) rectangle (axis cs: 2.650000e+01,2.750000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 0,0) -- (axis cs: 29,0);
\draw[-,red,line width=0.5mm] (axis cs: 29,5) -- (axis cs: 29,0);
\draw[-,red,line width=0.5mm] (axis cs: 0,5) -- (axis cs: 29,5);
\draw[-,red,line width=0.5mm] (axis cs: 0,5) -- (axis cs: 0,0);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.250000e+00) -- (axis cs: 2.650000e+01,2.250000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.650000e+01,2.750000e+00) -- (axis cs: 2.650000e+01,2.250000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.750000e+00) -- (axis cs: 2.650000e+01,2.750000e+00);
\draw[-,red,line width=0.5mm] (axis cs: 2.500000e+00,2.750000e+00) -- (axis cs: 2.500000e+00,2.250000e+00);
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-80.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-81.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-82.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-83.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-84.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-85.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-86.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-87.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-88.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-89.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-90.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-91.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-92.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-93.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-94.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-95.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-96.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-97.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-98.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-99.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-100.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-101.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-102.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-103.txt};
\addplot+[no marks,blue,fill,smooth,solid,line width=0.5] plot file {\relincludepath Data/Datafile-104.txt};

